A General Analysis Framework of Lower Complexity Bounds for Finite-Sum Optimization

This paper studies the lower bound complexity for the optimization problem whose objective function is the average of $n$ individual smooth convex functions. We consider the algorithm which gets access to gradient and proximal oracle for each individual component. For the strongly-convex case, we prove such an algorithm can not reach an $\varepsilon$-suboptimal point in fewer than $\Omega((n+\sqrt{\kappa n})\log(1/\varepsilon))$ iterations, where $\kappa$ is the condition number of the objective function. This lower bound is tighter than previous results and perfectly matches the upper bound of the existing proximal incremental first-order oracle algorithm Point-SAGA. We develop a novel construction to show the above result, which partitions the tridiagonal matrix of classical examples into $n$ groups. This construction is friendly to the analysis of proximal oracle and also could be used to general convex and average smooth cases naturally.

==> spp.tex <==
\section{Saddle-point Problems}
Consider a SPP
\begin{align}
    \min_{\vx \in \sR^m} \max_{\vy \in \sR^m} ~ \varphi(\vx, \vy) 
    = \frac{\mu}{2} \norm{\vx}^2 - \sqrt{\frac{L^2 - 2\mu^2}{8}} \inner{\B^{\top} \vx - \ve_{m}}{\vy} - \frac{\mu}{2} \norm{\vy}^2.
\end{align}

We have 
\begin{align*}
    \varphi(\vx, \vy) = \frac{\mu}{2} \norm{\vx}^2 - \frac{\mu}{2} \norm{\vy}^2 
    - \sqrt{\frac{L^2 - 2\mu^2}{8}} \left( \sum_{i=1}^{m} x_i \vb_i^{\top} \vy - y_m \right)
\end{align*}
